Pathologies of Pre-trained Language Models in Few-shot Fine-tuning

Although adapting pre-trained language models with few examples has shown promising performance on text classification, there is a lack of understanding of where the performance gain comes from. In this work, we propose to answer this question by interpreting the adaptation behavior using post-hoc explanations from model predictions. By modeling feature statistics of explanations, we discover that (1) without fine-tuning, pre-trained models (e.g. BERT and RoBERTa) show strong prediction bias across labels; (2) although few-shot fine-tuning can mitigate the prediction bias and demonstrate promising prediction performance, our analysis shows models gain performance improvement by capturing non-task-related features (e.g. stop words) or shallow data patterns (e.g. lexical overlaps). These observations alert that pursuing model performance with fewer examples may incur pathological prediction behavior, which requires further sanity check on model predictions and careful design in model evaluations in few-shot fine-tuning.

==> Makefile <==
### latex.makefile
# Author: Jason Hiebel

PROJECT = main

# This is a simple makefile for compiling LaTeX documents. The core assumption
# is that the resulting documents should have any parameters effecting
# rendering quality set to theoretical limits and that all fonts should be
# embedded. While typically overkill, the detriment to doing so is negligible.

# Targets:
#    default : compiles the document to a PDF file using the defined
#              latex generating engine. (pdflatex, xelatex, etc)
#    display : displays the compiled document in a common PDF viewer.
#              (currently linux = evince, OSX = open)
#    clean   : removes the obj/ directory holding temporary files

default: obj/$(PROJECT).pdf

display: default
	(${PDFVIEWER} obj/$(PROJECT).pdf &)


### Compilation Flags
CC = pdflatex 
PDFLATEX_FLAGS  = -halt-on-error -output-directory obj/

TEXINPUTS = .:obj/
TEXMFOUTPUT = obj/


### File Types (for dependancies)
TEX_FILES = $(shell find . -name '*.tex' -or -name '*.sty' -or -name '*.cls')
BIB_FILES = $(shell find . -name '*.bib')
BST_FILES = $(shell find . -name '*.bst')
IMG_FILES = $(shell find . -path '*.jpg' -or -path '*.png' -or \( \! -path './obj/*.pdf' -path '*.pdf' \) )


### Standard PDF Viewers
# Defines a set of standard PDF viewer tools to use when displaying the result
# with the display target. Currently chosen are defaults which should work on
# most linux systems with GNOME installed and on all OSX systems.

UNAME := $(shell uname)

ifeq ($(UNAME), Linux)
PDFVIEWER = evince
endif

ifeq ($(UNAME), Darwin)
PDFVIEWER = open
endif


### Clean
# This target cleans the temporary files generated by the tex programs in
# use. All temporary files generated by this makefile will be placed in obj/
# so cleanup is easy.

clean::
	rm -rf obj/

### Core Latex Generation
# Performs the typical build process for latex generations so that all
# references are resolved correctly. If adding components to this run-time
# always take caution and implement the worst case set of commands.
# Example: latex, bibtex, latex, latex
#
# Note the use of order-only prerequisites (prerequisites following the |).
# Order-only prerequisites do not effect the target -- if the order-only
# prerequisite has changed and none of the normal prerequisites have changed
# then this target IS NOT run.
#
# In order to function for projects which use a subset of the provided features
# it is important to verify that optional dependancies exist before calling a
# target; for instance, see how bibliography files (.bbl) are handled as a
# dependency.

obj/:
	mkdir -p obj/

obj/$(PROJECT).aux: $(TEX_FILES) $(IMG_FILES) | obj/
	$(CC) $(PDFLATEX_FLAGS) $(PROJECT)

obj/$(PROJECT).bbl: $(BIB_FILES) | obj/$(PROJECT).aux
	bibtex obj/$(PROJECT)
	$(CC) $(PDFLATEX_FLAGS) $(PROJECT)

obj/$(PROJECT).pdf: obj/$(PROJECT).aux $(if $(BIB_FILES), obj/$(PROJECT).bbl)
	$(CC) $(PDFLATEX_FLAGS) $(PROJECT)
	grep --color auto -e "Warning" obj/$(PROJECT).log


==> relate.tex <==
\section{Related Work}
\label{sec:relate}
Pre-trained language models like BERT \citep{devlin-etal-2019-bert}, RoBERTa \citep{liu2019roberta} and GPT-3 \citep{NEURIPS2020_1457c0d6} have shown remarkable adaptation performance on downstream tasks due to their learning ability and prior knowledge gained during pre-training \citep{gururangan-etal-2020-dont}. 
Moreover, this adaptation power is also expected when the number of task-specific examples is limited, which is likely to happen in the real world, such as data privacy or expense constraints. 
To fulfill this goal, much effort has been put into improving model adaptation performance in few-shot or zero-shot settings \citep{schick-schutze-2021-exploiting, gao-etal-2021-making, chen-etal-2021-revisiting}.
However, there is a lack of work on analyzing model adaptation behavior or explicit evidence supporting that the performance gain is truly based on useful information.

\citet{utama2021avoiding} disclosed that models obtained from few-shot prompt-based fine-tuning tend to adopt inference heuristics (i.e. lexical overlap) to make predictions on sentence pair classification tasks. 
\citet{ma2021issues} revealed the performance variance of entailment-based models across zero-shot text classification tasks. 
\citet{zhao2021calibrate} discovered the instability of model performance towards different prompts in few-shot learning. 
These works either focused on a specific scheme (e.g. prompt) in few-shot learning or a common problem (e.g. lexical overlap) associated with a type of sentence pair classification tasks. 
Differently, we study a more general adaptation process of pre-trained language models in standard few-shot fine-tuning. 
Besides, we first explain model few-shot adaptation behavior via post-hoc explanations, which sheds light on future research on few-shot fine-tuning or learning. 

